AMR-RE: Abstract Meaning Representations for Retrieval-Based In-Context Learning in Relation Extraction

Existing in-context learning (ICL) methods for relation extraction (RE) often prioritize language similarity over structural similarity, which can lead to overlooking entity relationships. To address this, we propose an AMR-enhanced retrieval-based ICL method for RE. Our model retrieves in-context examples based on semantic structure similarity between task inputs and training samples. Evaluations on four standard English RE datasets show that our model outperforms baselines in the unsupervised setting across all datasets. In the supervised setting, it achieves state-of-the-art results on three datasets and competitive results on the fourth.

==> 0_abstract_old.tex <==
\begin{abstract}

In-context learning (ICL) for relation extraction (RE) has achieved promising performance, but still faces a significant challenge regarding the quality of ICL demonstrations. 
Existing approaches focus on language similarity, and often ignore structural similarity. This might cause the models to overlook obvious relationships between entities in a text. Abstract Meaning Representations (AMR) provide a structured and more explicit semantic representation of relationships and entities. 
%Existing models struggle to overcome the issue since they directly model the context using the language model, which underestimates the semantic associations between entities. 
In this work, we propose an AMR-enhanced ICL method for RE. We explore the AMR structure generated for a sentence at the subgraph level (shortest AMR path).
%, explicitly modeling the semantic associations between entities. 
We demonstrate that two settings (fine-tuned or non-fine tuned) benefit from the fine-grained AMR's semantic structure. We evaluate our model on four RE datasets. Our results show that our model can outperform the GPT-based baselines, and achieve SOTA performance on two of the datasets, and competitive performance on the other two. 

%(1) \FWNAME can benefit from the trimmed AMR graph and self-supervised training and consistently shows improvements to sentence embedding-based baselines; (2) fine-tuned ICL framework achieves SOTA on Semeval and TB-Desnse, which incorporates AMR graph information to enrich the RE representation for selecting high-quality ICL demonstrations.

\end{abstract}

==> 1_intro_old.tex <==
\section{Introduction}
%% Lis: just drafting some random sentences, pls ignore if they don't make sense for your paper
%the story will change, depending on the focus of the paper

%Large language models (LLMs) such as GPT-3  \cite{mann2020language} have shown remarkable capabilities across a range of downstream tasks in natural language processing (NLP) (\citealp{chowdhery2023palm}; \citealp{rae2021scaling}; \citealp{hoffmann2022training}), However, fine-tuning these LLMs presents challenges due to their closed-source nature and high training costs. Therefore, there is a need for more cost-efficient strategies to adapt LLMs to various use contexts. 
%Recently, a new paradigm known as in-context learning (ICL) \citep{brown2020language} has emerged. 
Large language models (LLMs) have shown the remarkable ability for in-context learning (ICL) on many nlp tasks, such as natural language inference \citep{he2023using} and text classification \citep{sun-etal-2023-text}.   
ICL enables LLMs to perform new tasks without updating any of the model's weights, by simply providing the model with a few demonstrations of the task, along with the desired outputs \cite{brown2020language}. 

%However, one limitation of LLMs is their dependence on unstructured text, which occasionally leads these models to overlook apparent logical entailments or hallucinate incorrect conclusions \cite{zhang2023hallucination}.
However, downstream tasks that require high precision, such as relation extraction (RE), can still be challenging for ICL. 
%Relation extraction consists of finding a predefined semantic relation among pairs of entities mentioned in text.
RE consists of finding a predefined semantic relation among entity pairs mentioned in the input sentence, or NULL if no relation is found \cite{wan-etal-2023-gpt}. 
%In ICL settings, the quality of ICL demonstrations is vital for the model's performance. Existing methods adopt manual selection \cite{chan-etal-2024-exploring}, sentence embeddings \cite{ma-etal-2023-large}, or fine-tuned RE representation \cite{wan-etal-2023-gpt} to find relevant demonstrations. 
Relations between entity pairs are often implicitly expressed in text. In addition to entity mentions, entities are associated with their arguments, which in turn relate to other semantic elements \cite{hu-etal-2023-semantic}.Existing ICL methods for RE underestimate the semantic associations, as they commonly rely on entity mentions or overall sentence semantics for representation (\citealp{han2023information}; \citealp{wan-etal-2023-gpt}).  %Based on this, we propose to explicitly model these associations that can inductively represent the relations by incorporating fine-grained entity-associated semantic structures.
% sentence embedding -> sentence + entity -> shortest path (semantic + entity + association)

%Word meanings are sometimes best represented as relations among referents, including both individuals and events \cite{bender2022linguistic}. 
Abstract Meaning Representation (AMR) \cite{banarescu2013abstract} represents relations in a semantic graph structure, with nodes corresponding to semantic elements in the text (e.g., events, entities, concepts) and edges indicating the relations between them. AMR graphs provide precise descriptions of entities by incorporating their arguments and semantic roles, making it suitable for the RE task (\citealp{hu-etal-2023-semantic}; \citealp{zhang-ji-2021-abstract}; \citealp{gururaja-etal-2023-linguistic}). %For example, an example is shown in Figure \ref{fig:samples} with its relation and entity-associated semantic structure which is extracted from its AMR graphs, this concise structure can inductively indicate the "BEFORE" relation between "genocide" and "said".
Figure \ref{fig:samples} exemplifies the AMR graph representation of an input sentence. Its concise relations and the derived AMR graph intuitively indicate the "Content-Container" relation between the entities "rum" and "bottle".

%AMR naturally captures the hierarchical relations between entities in text, making it favorable for the relation extraction task.

%the essence of texts by encoding them in a semantic graph structure, where nodes indicate events, entities, concepts, and other semantic elements, while edges with semantic roles describe the associations among the semantic elements.

%is a semantic representation language that effectively captures the essence of texts by where the nodes indicate events, entities, concepts, and other semantic elements, while edges with semantic roles describe the associations among semantic elements.
%encoding abstract-level semantic information, including named entities, negations, coreferences, and modalities. (rephrase this later)

%tries to capture many aspects of meaning in a single simple data structure \cite{schneider-etal-2015-logic}. 

%Each sentence is represented as a rooted, directed, acyclic graph with labels on edges (relations) and nodes (concepts).

% Maybe include this later
%However, the intersection of AMR and LLMs has been relatively understudied. 
%(Mention some related work)
%...

%%Recent studies have shown that LLMs possess a strong capability for in-context learning, being able to extract and leverage valuable information from retrieved knowledge to rectify nonfactual claims they previously generated \cite{zhang2023hallucination}. Graph-structured knowledge can be a flexible way to provide LLMs with such retrieved knowledge.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figs/sample.png}
  \caption{Overview of the shortest AMR path construction.}
  \label{fig:samples}
\end{figure}

We hypothesize that the AMR's explicit representation of semantic structures can improve the quality of few-shot demonstrations, and further enhance LLMs' ICL ability for RE. To exploit the potential utilization of AMR graphs for RE in ICL, we propose two novel semantic structure-enhanced ICL frameworks: one that explores the AMR structure generated for a sentence at the subgraph level (shortest AMR path) , and another that explores the full AMR structure generated for a sentence. In both cases, we demonstrate that all settings benefit from the fine-grained AMR's entity structure.
%(1) \textbf{T}rimmed \textbf{A}MR \textbf{G}raph representation-based ICL (\textbf{TAG-ICL}); (2) \textbf{F}ine-\textbf{T}uned \textbf{S}tructure representation-based ICL (\textbf{FTS-ICL}). 
We evaluate our methods on four standard RE datasets. 
%: SemEval, SciERC, TB-Dense and ACE05. 
Our results indicate that our model consistently achieves higher F1 scores than other sentence embedding-based ICL baselines; incorporating supervised fine-tuning and LLM's capability can even outperform SOTA baselines on two of the evaluated datasets. We further observe that our method can achieve promising performance in a more cost-efficient manner.
%More specifically, we propose a method for reasoning over AMR-semantic representations for use by LLMs during ICL. We show that our method can improve the quality of the retrieved ICL demonstrations for the RE task, and improve the model's overall performance. 


% Specifically, our contributions are:
% %our method allows the LLMs to outperform the SOTA in RE tasks in a more cost-efficient manner?
% 1) we propose two novel semantic structure representation-enhanced ICL frameworks, \FWNAME and \FWFTNAME, which both benefit from fine-grained AMR graph representations;
% % They can select more relevant ICL demonstrations by explicitly capturing the associations between entities for RE
% 2) according to experimental results on four RE datasets, \FWNAME consistently achieves higher F1 scores than other sentence embedding-based ICL baselines; \FWFTNAME incorporating supervised fine-tuning and LLM's capability outperforms SOTA baselines on two datasets; 
% 3) we implement ablation studies, and the results show that our method can achieve promising performance in a more cost-efficient manner.

% Our method avoids the need for modifying LLMs internally or using additional knowledge bases, making it a flexible plug-and-play and efficient RE model.

==> 2_method_old.tex <==
\begin{figure*}[t]
  \includegraphics[width=\linewidth]{figs/main.png} 
  \caption {An overview of our proposed method. Given an input, we first adopt two distinct AMR-enhanced demonstration retrieval methods to select proper demonstrations from the training set. Subsequently, all retrieved demonstrations are included in the prompt construction to facilitate the prediction.}
  \label{fig:main}
\end{figure*}

\section{The \MNAME~Model}
% : \DNAME \todo[inline]{please change  the DNAME value (main tex file) if you change the name of your model}
In this section, we first show the prompt construction for formalizing RE into a language generation task
(Section \ref{prompt}). Then we introduce the AMR-enhanced demonstration retrieval frameworks that benefit from the fine-grained relational semantic structure information in two settings: non-fine tuned (Section \ref{sec:nonft}) and fine-tuned (Section \ref{sec:ft}) ICL frameworks. An overview of our proposed method is shown in
Figure \ref{fig:main}.

\subsection{Task Definition}
Given a set of pre-defined relation classes $\mathbb{R}$, relation extraction aims to predict the relation $y \in \mathbb{R}$ between the given pair of subject and object entities $(e_{sub}, e_{obj})$ within the input context $\mathbf{C}$, or if there is no pre-defined relation between them, predict $y = \text{NULL}$.

\subsection{Prompt Construction\label{prompt}}
Following \citet{wan-etal-2023-gpt}, we construct a prompt for each test example. Each prompt consists of the following three components:

%\begin{description}[leftmargin=*]
    %\item[Instructions]
    
    \noindent\textbf{Instructions}: We provide a precise description of the RE task and a set of pre-defined relation classes. The model is required to output the relation corresponding to these predefined classes; if the relation does not belong to any of these classes, the model will output NULL.
    
    %\item[ICL Demonstrations]
    \noindent\textbf{ICL Demonstrations}: Given one test example, We search $k$-nearest neighbor ($k$NN) demonstrations via two different frameworks: non fine-tuned \FWNAME (Section \ref{sec:nonft}) and fine-tuned \FWFTNAME (Section \ref{sec:ft}). All demonstrations are included in the prompt.

    %\item[Test Input] 
    \noindent\textbf{Test Input}: We provide the test input in the same format as ICL Demonstrations, and GPT is expected to output the relation.

%\end{description}

\subsection{AMR Graph}
We propose to explicitly model semantic associations between two entities by integrating semantic structure for RE. To get explicit semantic structures from texts we adopt an off-the-shelf AMR parser\footnote{\url{https://github.com/IBM/transition-amr-parser}} to process the sentence into an AMR graph. We parse the input sentence into an AMR graph $G=\{V,E,R\}$, where $V$, $E$, $R$ are the sets of nodes, edges and relation types, respectively. In AMR graph $G$, the labeled edge $(u,r,v) \in E$, where $u, v \in V$ and $r \in R$ is a relation type, means that there is an edge labeled as $r$ from node $u$ to node $v$.

\subsection{Shortest AMR Path Representation for ICL \label{sec:nonft}}
Recent works (\citealp{jimenez-gutierrez-etal-2022-thinking}; \citealp{liu-etal-2022-makes}; \citealp{wan-etal-2023-gpt}) adopt the $k$NN method to retrieve the most similar examples in the training set as the few-shot demonstrations for each test input using sentence embedding obtained by the PLM. Since $k$NN relies on the choice of the embedding space, previous works use various methods, such as SimCSE \citep{gao-etal-2021-simcse}, Sentence-BERT \citep{reimers-gurevych-2019-sentence}, and fine-tuned relation representation \citep{wan-etal-2023-gpt} to improve performance on the RE task.

As relation extraction focuses on pair-wise entities, existing methods focus on entire sentence similarity or only capture implicit associations between two entities by directly modeling the texts with pre-trained language model (PLM), which underestimates the explicit semantic associations. In this section, we introduce \FWNAME, a shortest AMR path (SAP) representation based demonstration retrieval method that leverages fine-grained semantic graphs to enhance the quality of retrieved demonstrations.

\subsubsection{Shortest AMR Path Representation}
In an AMR graph, we hypothesize that the shortest path between two entities consistently contains information that reflects their semantic relationship. Therefore, we hypothesize that SAP is the most informative subgraph in the AMR for representing semantic relations. Formally, SAP is defined as $G_{p}=\{V_{p},E_{p},R_{p}\}$, where $V_{p}\in V, E_{p}\in E, R_{p}\in R$. Figure \ref{fig:samples} shows an overview of the SAP construction. Consequently, the TAG benefits not only from the information of the entities but also from the semantic associations between them.
% \footnote{The shortest path is computed by NetworkX in \url{https://networkx.org/}}
% Formally, a shortest path between two entities can be denoted as $[(v^{e1}_1,r_1,v_2,r_2,\cdot\cdot\cdot,v_{l-1}, r_{l-1},v^{e2}_l)]$, where $l$ is the length of the path; $v_i$ denotes the $i$-th node in the path, while $v_1$ and $v_l$ represent two entities, respectively; and $r_i$ denotes the representation of the relation $i$.

We adopt a graph encoder to effectively assess the similarity between two AMR subgraphs. In this work, we adopt AMRSim \cite{shou-lin-2023-evaluate}, a PLM that was self-supervised trained on AMR graphs, as the graph encoder. Given an AMR graph $G=[(u_1,r_1,v_1),\cdot\cdot\cdot,(u_n,r_n,v_n)]$, it will be first converted into an unlabeled graph $G=[(u_1,r_1),(r_1,v_1),\cdot\cdot\cdot,(u_n,r_n),(r_n,v_n)]$ by replacing each edge $(u,r,v)$ with two unlabeled edges $\{(u,r),(r,v)\}$. Then $G$ is linearized by a depth-first traversal algorithm $G=[u_1,r_1,v_1,\cdot\cdot\cdot,u_n.r_n,v_n;\mathcal{A}]$, where $\mathcal{A}$ is the adjacency matrix. $G$ will be fed to AMRSim to obtain the graph representations $h_{graph}$.

\begin{equation}
h_{graph} = \text{AMRSim}([u_1,r_1,v_1,\cdot\cdot\cdot,v_n]; \mathcal{A})
\end{equation}

\subsubsection{Self-supervised Training for Shortest AMR Path Representation}
% AMRSim requires the sequence input data. Therefore, given a TAG $G_{T}=\{V_{T},E_{T},R_{T}\}$, $G_{T}$ is first preprocessed into an unlabeled graph $G_{T}^{'}=\{V_{T}^{'}, E_{T}^{'}\}$ by replacing each edge $(u,r,v)$ with two unlabeled edges $\{(u,r),(r,v)\}$ for facilitating the model to learn from edges' semantics. Then $G_{T}^{'}$ is linearized by a depth-first traversal algorithm. 

% \subsubsection{Self-supervised Training for Trimmed AMR Graph \label{sec:sst}}
As mentioned, the original AMRSim is a self-supervised approach for optimizing the representation of the entire AMR graph. In our work, we adapt this approach to the subgraph level to obtain representations of the shortest AMR paths. 

We adopt the self-supervised training process Contrastive Tension (CT; \citealp{carlsson2021semantic}) on SAP to ensure that the model accurately performs on such structures following \citet{shou-lin-2023-evaluate}. The training objective is to maximize the dot product between positive pairs $(G_{p},G_{p}^{+})$ while minimizing the dot product between negative pairs $(G_{p},G_{p}^{-})$. For each randomly selected SAP $G_{p}$, we use $G_{p}^{+}=G_{p}$ to create a positive pair. Then, we construct negative instances by pairing $G_p$ with $K$ randomly sampled different graphs. The $K+1$ instances are included in the same batch. The training contrastive loss $\mathcal{L}$ is binary cross-entropy between the similarity scores and labels.
\begin{equation}
\mathcal{L} =
\begin{cases} 
-\log \sigma(h_{graph}\cdot h_{graph}^{+})\\%, & \text{if } \hat{G_T}=G_{T}^{+} \\
-\log \sigma(1-h_{graph}\cdot h_{graph}^{-})%,  & \text{if } \hat{G_T}=G_{T}^{-}
\end{cases}
\end{equation}

where $\sigma$ refers to the Logistic function; $h_{graph}$ is the graph representation. After CT on SAP, we employ the updated model for computing the similarity.

\subsection{Fine-tuned AMR-enhanced Representation for ICL \label{sec:ft}}
Considering that using fine-tuned relation representation can achieve promising performance for RE in ICL settings \citep{wan-etal-2023-gpt}, we adopt a fine-tuned model for retrieving ICL demonstrations. As current RE models that capture context and entity information show their effectiveness, we combine AMR graph and text input into a single model architecture to capture both semantics and structure connections of the input data, following previous works (\citealp{schrack-etal-2022-amr}; 
 \citealp{li-etal-2022-cross-domain}; \citealp{gururaja-etal-2023-linguistic}).

% \noindent\textbf{Textual-based model:} Existing RE models \citep{zhong-chen-2021-frustratingly} use special marker tokens to highlight the entities. We concatenate the context representations of $h_{e1}, h_{e2}$, where $h_{e1}, h_{e2}$ are the hidden representation of two beginning entity markers, respectively. We then feed this concatenated representation into a two-layer MLP with a ReLU activation between layers, before applying softmax for the classification.
 % For instance, "Good to have \underline{you} with \underline{us}.", the modified input is "[CLS] Good to have [SUB\_PER] \underline{you} [/SUB\_PER] with [OBJ\_ORG] \underline{us} [/OBJ\_ORG]. [SEP]", where “PER” is the entity type if provided.

To better utilize both AMR graph and textual information, we propose to train a feature fusion model. In this setting, the sentence and shortest AMR path of input are fed to the textual-based model and graph encoder, respectively. We employ a marker-based approach PURE \citep{zhong-chen-2021-frustratingly} to encode a sentence by adding special entity markers surrounding two entities. We employ AMRSim to model the shortest AMR path. After computing token embeddings of two special markers $h_{[SUB]}, h_{[OBJ]}$ and graph representations $h_{grpah}$, we define AMR-enhanced Representation as $h_{AMR+} = h_{grpah} \oplus h_{[SUB]} \oplus h_{[OBJ]}$. We then feed $h_{AMR+}$ into a two hidden layers multi-layer perceptron (MLP) network with a ReLU activation between the layers, before applying softmax for the classification. The AMR-enhanced representation $h_{AMR+}$, which benefits from both textual and AMR information, can potentially overcome the limitation of ICL.

==> 4_results_old.tex <==
\section{Results}
\input{tables/main_results}
\input{tables/ablation_cl}

\subsection{Main Results}
Table \ref{table:mainresults} presents the experimental results on the RE datasets. \textbf{\FWNAME} denotes our TAG representation-based ICL and \textbf{\FWFTNAME} denotes our fine-tuned structure representation-based ICL. Compared with baselines utilizing non fine-tuned retrievers, we can observe that \FWNAME consistently outperforms baselines on all four datasets. This shows the effectiveness and generality of TAG representation for selecting more relevant ICL demonstrations. \FWFTNAME outperforms baselines with fine-tuned retrievers on three datasets (SemEval, SciERC, TB-Dense), it achieves $0.51\%$,  $0.26\%$, and $1.77\%$ improvement, respectively. The results indicate that the fine-tuned structure representation benefits from both structural and semantic information. Consequently, \FWFTNAME achieves SOTA performance on the SemEval and TB-Dense datasets while delivering competitive results on the SciERC and ACE05 datasets.

\subsection{Ablation Studies}
We perform the ablation studies on CT and fusion feature, the results are shown in Table \ref{table:assst}. 

\noindent\textbf{Impact of the self-supervised training}: We conduct experiments without the additional training phase to investigate the effect of CT on SAP. The results indicate that CT on SAP significantly improves performance, demonstrating that CT can enhance the graph encoder's modeling capability of SAP. 

\noindent\textbf{Impact of fusion feature}: We conduct experiments To illustrate the effect of the fusion feature in fine-tuned settings. Although fine-tuned graph representation performs worse than sentence embedding, it shows that the model incorporating AMR better captures the relation than the text-only system.

\noindent\textbf{Effect of the Number of Few-shot Demonstrations}
We investigated the effect of the number of few-shot demonstrations on performance. Figure \ref{fig:kshot} shows the results: \FWNAME achieves a more significant improvement with fewer demonstrations compared to non fine-tuned baselines, indicating that our method requires shorter prompt for achieving promising performance; \FWFTNAME achieves better performance throughout all $k$-shots than GPT-RE\_FT, demonstrating the effectiveness of incorporating AMR graph.

\begin{figure}[t]
  \includegraphics[width=\columnwidth]{figs/kshot.png }
  \caption{Performance for the different number of few-shot examples on TB-Dense using \textsf{gpt-3.5-turbo}.}
  \label{fig:kshot}
\end{figure}

==> 5_unsupervised.tex <==
\section{\NONREFTNAME~ \MNAME} \label{sec:unsup_model}

Even though \MNAME\ delivers strong results on the four datasets, the \REFTNAME~retriever demands extensive annotated RE data and substantial computational resources. We also suspect that the fully supervised setting is nearly saturated, leaving limited room for substantial advances. To address these limitations, we evaluate our approach in the more challenging \NONREFTNAME~ setting. \textcolor{red}{We propose a simple yet effective approach to investigate the generality and robustness of \MNAME. Our model retrieves examples using only AMR graph embeddings from \AMRSIMNAME, which means $R_{rel}=R_{graph}$. Note that \AMRSIMNAME~ is only self-supervised on the corpus without annotated relation labels.}

\subsection{\NONREFTNAME~Experiments}
We align most of the experiment settings with Section \ref{sec:exp}. For a fair comparison, we implement three baselines with \NONREFTNAME~ Retrievers: 1) \textit{GPT-Random:} we randomly select few-shot ICL demonstrations with additional constraints to ensure a more uniform label distribution. This approach has been shown to be more effective than the vanilla random method \cite{wan-etal-2023-gpt}; 2) \textit{GPT-Sent:} we follow \citet{bioiclre} to retrieve $k$NN demonstrations with SimCSE~\cite{gao-etal-2021-simcse}, which is widely used sentence embedding model.
% we adopt SimCSE \citep{gao-etal-2021-simcse}, a widely used sentence similarity model for demonstration retrieval; 
3) \textit{GPT-RE\_Entity+:} we adopt the entity-prompted sentence embedding proposed by \citet{wan-etal-2023-gpt} that incorporates both the entity pair and contextual information for retrieval.

\subsection{Results in the \NONREFTNAME~Setting}
Table \ref{table:mainresults_unsupervised} shows our results in the \NONREFTNAME~setting. \MNAME~consistently outperforms the baselines on all four datasets. These findings underscore the efficacy of AMR-enhanced graph RE representations in effectively capturing relational information. In particular, by focusing on the shortest AMR path, \MNAME~highlights core entities and the semantic relations between them, thereby reducing noise and providing clearer relational cues compared to conventional sentence-embedding-based approaches.

Overall, our results confirm that incorporating AMR into graph RE representations can lead to more accurate and robust relation extraction both in \REFTNAME~ and \NONREFTNAME~ settings.

==> 7_limitations.tex <==
\section{Limitations}
Although the AMR graph has proven effective for ICL on RE, it still faces several challenges when used in downstream tasks. The primary issue directly influencing RE is token alignment, which results in nodes and edges in AMR graphs lacking links back to the words in the text from which they are generated. This lack of token alignment limits the generalization of RE; for instance, if there are no nodes linking to entities, the AMR cannot be effectively implemented in such scenarios. Dependency parsers can serve as a potential alternative, as they do not require token alignment.

==> tables/ablation_cl_old.tex <==
% \begin{table}
%   \centering
%   \begin{tabular}{l|c|c|c}
%     \hline
%     \textbf{Dataset} &\textbf{\FWNAME} & w/o SST &$\Delta$\\
%     \hline
%     % \multicolumn{7}{c}{ICL w/ Non-fine-tuned Retriever} \\ \hline
%     SemEval & 68.63 & 65.37 & $-3.26\%$ \\ 
%     % \multicolumn{7}{c}{ICL w/ Fine-tuned Retriever} \\ \cline{1-7} 
%     TB-DENSE  & 27.39 & 24.37 & $-3.02\%$ \\
%     \hline
%   \end{tabular}
%   \caption{\label{table:assst}
%     \textbf{Ablation study on self-supervised training.} \textit{w/o SST} indicates that the retriever doesn't apply self-supervised training on entity-associated structures. We show the $10$-shot results from \textsf{gpt-3.5-turbo}.
%   }
% \end{table}
\begin{table}
\small
  \centering
  \begin{tabular}{l|c|c}
    \hline
    \textbf{Dataset} &\textbf{SemEval} & \textbf{SciERC}\\
    \hline
    \multicolumn{3}{c}{ICL w/ Non fine-tuned Retriever} \\ \hline
    \FWNAME & \textbf{84.68} & \textbf{27.57} \\
    \quad\textit{w/o CT} & 81.67 & 25.39 \\  \hline
    \multicolumn{3}{c}{ICL w/ Fine-tuned Retriever} \\ \hline
    \FWFTNAME & \textbf{91.97} & \textbf{67.41} 
    \\
    \quad\textit{w/o SentEmb} & 89.71 & 66.34  \\
    \quad\textit{w/o AMR} & 91.46 & 67.15 \\
    \hline
  \end{tabular}
  \caption{\label{table:assst}
    \textbf{Ablation study.} \textit{w/o CT} indicates that the retriever does not apply additional CT. \textit{w/o AMR} indicates that the retriever doesn't incorporate AMR graph for fine-tuning. We show the $10$-shot results from \textsf{gpt-4}.
  }
\end{table}

==> tables/main_results_old.tex <==
% \begin{table*}
%   \centering
%   \small 
%   \begin{tabular}{l|c|c|c|c|c|c}
%     \hline
%     \textbf{Method}           & \textbf{Retriever} & \textbf{GPT} &\textbf{SemEval} & \textbf{SciERC}  & \textbf{TB-DENSE} & \textbf{ACE05}  \\
%     \hline
%     \multicolumn{7}{c}{ICL w/ Non finetuned Retriever} \\ \hline
%     GPT-Random       & -      & 3.5-turbo     & 52.05 &  17.35  &22.97  &6.95                      \\ 
%     GPT-Sent     & SimCSE  & 3.5-turbo       & 65.37   &21.64   &23.21  &5.46                  \\ 
%     \multirow{2}{*}{GPT-RE\_Entity+}       & \multirow{2}{*}{SimCSE}   & 3.5-turbo     & 66.21 & 21.90 & 23.53  &10.07                       \\
%     \multirow{2}{*}{}  &\multirow{2}{*}{} & 4    &80.25  & 26.15 & 31.19 & 13.10\\ 
%     \multirow{2}{*}{\FWNAME (Ours)}       & \multirow{2}{*}{\DNAME}   & 3.5-turbo     & 68.63  & 22.73 &27.39  &11.32           \\
%     \multirow{2}{*}{}  &\multirow{2}{*}{}  & 4  & \textbf{84.68} & \textbf{27.57} & \textbf{35.10} & \textbf{14.65}  \\ \hline
%     \multicolumn{7}{c}{ICL w/ Fine-tuned Retriever} \\ \cline{1-7}
%     \multirow{2}{*}{GPT-RE\_FT}       & \multirow{2}{*}{PURE}   & 3.5-turbo        & 89.73  & 64.53 & 65.64  &  66.81                  \\
%     \multirow{2}{*}{}  &\multirow{2}{*}{}  & 4    &91.46  & 67.15 & 67.58 &  \textbf{68.59} \\ 
%     \multirow{2}{*}{\FWFTNAME (Ours)}       & \multirow{2}{*}{\FTNAME}   & 3.5-turbo        & 90.25  & 64.93 & 66.08 & 65.27                       \\
%     \multirow{2}{*}{}  &\multirow{2}{*}{}  & 4    &\textbf{91.89}  & \textbf{67.81}  & \textbf{68.69} & 66.80\\
%     \hline
%   \end{tabular}
%   \caption{\label{table:mainresults}
%     \textbf{Main results on four RE datasets.} All results are given by Micro-F1 in $10$-shot ICL settings.
%   }
% \end{table*}

\begin{table*}
  \centering
  \small 
  \begin{tabular}{l|c|c|c|c|c}
    \hline
    \textbf{Method}           & \textbf{GPT} &\textbf{SemEval} & \textbf{SciERC}  & \textbf{TB-DENSE} & \textbf{ACE05}  \\
    \hline
    \multicolumn{6}{c}{ICL w/ Non finetuned Retriever} \\ \hline
    GPT-Random            & 3.5-turbo     & 52.05 &  17.35  &22.97  &6.95                      \\ 
    GPT-Sent       & 3.5-turbo       & 65.37   &21.64   &23.21  &5.46                  \\ 
    \multirow{2}{*}{GPT-RE\_Entity+}          & 3.5-turbo     & 66.21 & 21.90 & 23.53  &10.07                       \\
    \multirow{2}{*}{}  & 4    &80.25  & 26.15 & 31.19 & 13.10\\ 
    \multirow{2}{*}{\FWNAME (Ours)}         & 3.5-turbo     & 68.63  & 22.73 &27.39  &11.32           \\
    \multirow{2}{*}{}    & 4  & \textbf{84.68} & \textbf{27.57} & \textbf{35.10} & \textbf{14.65}  \\ \hline
    \multicolumn{6}{c}{ICL w/ Fine-tuned Retriever} \\ \hline
    \multirow{2}{*}{GPT-RE\_FT}          & 3.5-turbo        & 89.73  & 64.53 & 65.64  &  66.81                  \\
    \multirow{2}{*}{}    & 4    &91.46  & 67.15 & 67.58 &  \textbf{68.59} \\ 
    \multirow{2}{*}{\FWFTNAME (Ours)}         & 3.5-turbo        & 90.25  & 64.93 & 66.08 & 65.27                       \\
    \multirow{2}{*}{}    & 4    &\textbf{91.97}  & \textbf{67.41}  & \textbf{69.15} & 66.80\\
    \hline
  \end{tabular}
  \caption{\label{table:mainresults}
    \textbf{Main results on four RE datasets.} All results are given by Micro-F1 in $10$-shot ICL settings. For a fair comparison, all the results are produced by ourselves. 
  }
\end{table*}

==> tables/main_results_unsup.tex <==
% \begin{table*}
%   \small
%   \centering
%   \begin{tabular}{l|c|c|c|c|c|c}
%     \hline
%     \textbf{Method} &\textbf{Retriever}  &\textbf{SemEval($\Delta$\%)} & \textbf{TB-DENSE($\Delta$\%)} & \textbf{SciERC($\Delta$\%)}  & \textbf{ACE05($\Delta$\%)}&\textbf{Avg}  \\
%     \hline
%     GPT-Random  &-   & 67.83 &  22.03  &16.48  &9.73 & 29.02                     \\ 
%     GPT-Sent   &SimCSE      & 77.64   &28.73   &21.60  &10.04 & 34.50                 \\ \hline
%     GPT-RE\_Entity+  &SimCSE        &  80.25 (-)  & 31.19 (-)  & 26.15 (-)   &13.10 (-)   & 37.67                   \\
    
%     \MNAME\textsubscript{\textit{\GENAME}} &\textit{\AMRSIMNAME}    &  81.40 ($\uparrow$ 1.4)  & \textbf{38.17 ($\uparrow$ 22.4)} &\textbf{$\mathbf{27.89^{\ast}}$ ($\uparrow$ 6.7)} & \textbf{$\mathbf{15.04^{\ast}}$ ($\uparrow$ 14.8)}   & 40.52  \\

%     \MNAME\textsubscript{\textit{\PENAME}} &\textit{\AMRSIMNAME}       &  \textbf{84.68 ($\uparrow$ 5.5)} & 35.64 ($\uparrow$ 14.3) & $27.56^{\ast}$ ($\uparrow$ 5.4) & $14.69^{\ast}$ ($\uparrow$ 12.1)    & \textbf{40.64}  \\
    
%     \hline
%   \end{tabular}
%   \caption{\label{table:mainresults_unsupervised}
%     \textbf{Main results in \textit{\NONREFTNAME}~setting.} \MNAME\textsubscript{\GENAME} and \MNAME\textsubscript{\PENAME} refer to the \textit{\GENAME} and \textit{\PENAME} graph representation setups, respectively, explained in Section \ref{sec:graph_enc}. The $\Delta$\% is the corresponding percentage of improvement gains compared with {GPT-RE\_Entity+}. The Avg column shows the average score for all datasets. The best results are in \textbf{bold}. $\ast$ denotes that this result is implemented by concatenation pooling, otherwise, mean pooling is used.
%   }
% \end{table*}

\begin{table*}
  \small
  \centering
  \begin{tabular}{l|c|c|c|c|c|c}
    \hline
    \textbf{Method} &\textbf{Retriever}  &\textbf{SemEval($\Delta$\%)} & \textbf{TB-DENSE($\Delta$\%)} & \textbf{SciERC($\Delta$\%)}  & \textbf{ACE05($\Delta$\%)}&\textbf{Avg}  \\
    \hline
    GPT-Random  &-   & 67.83 &  22.03  &16.48  &9.73 & 29.02                     \\ 
    GPT-Sent   &SimCSE      & 77.64   &28.73   &21.60  &10.04 & 34.50                 \\
    GPT-RE\_Entity+  &SimCSE        &  80.25 (-)  & 31.19 (-)  & 26.15 (-)   &13.10 (-)   & 37.67                   \\
    
    \MNAME~(Ours) &\textit{\AMRSIMNAME}    &  \textbf{\underline{84.68} ($\uparrow$ 5.5)}  & \textbf{38.17 ($\uparrow$ 22.4)} &\textbf{$\mathbf{27.89^{\ast}}$ ($\uparrow$ 6.7)} & \textbf{$\mathbf{15.04^{\ast}}$ ($\uparrow$ 14.8)}   & 41.45  \\
    
    \hline
  \end{tabular}
  \caption{\label{table:mainresults_unsupervised}
    \textbf{Main results in \textit{\NONREFTNAME}~setting.} We set the number of demonstrations to $k=10$. The $\Delta$\% is the corresponding score difference with GPT-RE\_FT. The Avg column shows the average score for all datasets. We align the annotations with Table \ref{table:mainresults}.
  }
\end{table*}
